Enhancing Low-resource Fine-grained Named Entity Recognition by Leveraging Coarse-grained Datasets

Named Entity Recognition (NER) frequently suffers from the problem of insufficient labeled data, particularly in fine-grained NER scenarios. Although $K$-shot learning techniques can be applied, their performance tends to saturate when the number of annotations exceeds several tens of labels. To overcome this problem, we utilize existing coarse-grained datasets that offer a large number of annotations. A straightforward approach to address this problem is pre-finetuning, which employs coarse-grained data for representation learning. However, it cannot directly utilize the relationships between fine-grained and coarse-grained entities, although a fine-grained entity type is likely to be a subcategory of a coarse-grained entity type. We propose a fine-grained NER model with a Fine-to-Coarse(F2C) mapping matrix to leverage the hierarchical structure explicitly. In addition, we present an inconsistency filtering method to eliminate coarse-grained entities that are inconsistent with fine-grained entity types to avoid performance degradation. Our experimental results show that our method outperforms both $K$-shot learning and supervised learning methods when dealing with a small number of fine-grained annotations.

==> method_old.tex <==
\section{Proposed method - OLD}
% inde

\subsection{Problem definition}
Given a sequence of tokens $\mathbf X = \{x_1,x_2, ..., x_n\}$, 
the task of NER is to assign a type $y\in$ to each toke

$\mathbf X^F = \{x^F_1,x^F_2, ..., x^F_n\}$ is a training sample of length $n$, $\mathbf Y^F = \{ y^F_1, y^F_2, ..., y^F_n\}$ is the corresponding label sequence of $\mathbf{X^F}$. 

Given a low-resource fine-grained dataset $\mathcal D_F = \{(\mathbf X^F_1,\mathbf Y^F_1), ..., (\mathbf X^F_l,\mathbf Y^F_{|D_F|})\}$, where $\mathbf X^F = \{x^F_1,x^F_2, ..., x^F_n\}$ is a training sample of length $n$, $\mathbf Y^F = \{ y^F_1, y^F_2, ..., y^F_n\}$ is the corresponding label sequence of $\mathbf{X^F}$. 



In this section, we first depict the overall training process in \cref{Overall Process}.
As shown in Figure \ref{fig: overall}, our approach demonstrates a training process that consists of two main datasets, a fine-grained dataset, and a coarse-grained dataset.
To utilize a coarse-grained dataset together, we introduce two main components: the F2C mapping matrix(\cref{F2C Mapping Matrix}), and the inconsistency filtering process(\cref{Inconsistency Filtering}).
% During the training process with the coarse-grained dataset, we introduce two key components: the F2C mapping matrix (\autoref{F2C Mapping Matrix}), and the inconsistent type filter (\autoref{Inconsistent Type Filter}).

%---------------------------이부분 빼기? 
% The shared purpose of the two components is to give a single model two kinds of datasets for enhancing hierarchical connections.
% 우리의 핵심 아이디어는 training동안 여러 데이터셋을 동시에 사용함으로써 datasets 사이의 label hierarchy를 직접적으로 반영하는 것이다
% The F2C mapping matrix is dedicated to mapping the hierarchy between fine-grained and coarse-grained types during the training phase. 
% This mapping process enables the model trained with differently-grained datasets.
% Mapping matrix는 두 데이터셋의 entity types를 매핑해 여러 데이터셋을 동시에 학습에 이용할 수 있도록 만든다.
% Afterward, we discuss the inconsistent type filter, which allows the filtering of noisy data in coarse-grained datasets that are ambiguous to map with fine-grained entity types. 
% Via this filter, we can mitigate entity type mismatch problems. 
% 이때, CG-dataset과 FG-Dataset 사이의 inconsistancy로 인해 noise information을 필터링해줄 수 있는 





\textit{Filtering Method}를 추가적으로 사용한다. 이를 통해 coarse-grained dataset이 가진 noisy한 정보를 필터링하여 FG-NER에 적합한 데이터만 유동적으로 사용할 수 있다.
%----------------------------

\subsection{Overall Process} \label{Overall Process}
We aim to directly reflect a two-level hierarchy by concurrently using differently-grained multiple datasets in a single model training. 
% 우리의 핵심 아이디어는 training동안 여러 데이터셋을 동시에 사용함으로써 datasets 사이의 label hierarchy를 직접적으로 반영하는 것이다. 
% 우리는 tag set 범위가 다른 데이터셋을 사용해 FG-NER을 해결하는 것을 목표로 한다.
Figure \ref{fig: overall} illustrates the overview of the fine-grained NER model training process using both the fine-grained and coarse-grained datasets.
% Fig 1은 FG-NER 모델 학습 시 FG-Dataset과 CG-dataset으로 각각 학습하는 과정을 보여준다.
The training with the fine-grained dataset is depicted in Figure \ref{fig: overall: a}.
%  Fig. 1(a)는 FG-dataset을 이용한 학습 과정이다.

Given a low-resource fine-grained dataset $\mathcal D_F = \{(\mathbf X^F_1,\mathbf Y^F_1), ..., (\mathbf X^F_l,\mathbf Y^F_l)\}$, where $\mathbf X^F = \{x^F_1,x^F_2, ..., x^F_n\}$ is a training sample of length $n$, $\mathbf Y^F = \{ y^F_1, y^F_2, ..., y^F_n\}$ is the corresponding label sequence of $\mathbf{X^F}$. 

We adopt $T^F = \{t_1^F, ..., t^F_f\}, (\forall y^F_i, y^F_j \in T^F)$ to represent the tag set of the fine-grained dataset, where $t$ is the number of fine-grained entity types.

$\mathbf X^F$ is fed into a \texttt{PLM} (pre-trained language model), \emph{e.g.}~\bert~\cite{BERT}, \roberta~\cite{RoBERTa}, to generate a contextual representations.
Then we get the label probability by using \textit{softmax}:
\begin{align}
\label{eq: plm}
\mathbf H = [h_1, ..., h_n ] = \texttt{PLM}([x^F_1, ..., x^F_n])    
\end{align}
\begin{align*}
p^F(y^F_i|x^F_i)= \text{\textit{softmax}} (Wh_i + b) 
\end{align*}
With the fine-grained dataset, the model is  trained by optimizing cross-entropy loss as follows:
\begin{align}
L_F = - \frac 1n \sum^n_{i=1} y^F_i \log (p^F(y^F_i|x_i))
\end{align}

Figure \ref{fig: overall: b} shows the training process with the coarse-grained dataset.
% Fig. 1(b)는 CG-dataset을 이용한 학습 프로세스를 보여준다.
Compared with prior works that use a task-specific classifier for each kind of dataset, we adopt only a single classifier for fine-grained NER.
% 이때 기존 연구와는 다르게, 각 데이터셋 별로 다른 top layer classifier를 사용하지 않고, FG-NER을 해결하기 위한 하나의 classifier만 사용한다.
We use high resource coarse-grained dataset $\mathcal D_C = \{(\mathbf X^C_1,\mathbf Y^C_1), ..., (\mathbf X^C_h,\mathbf Y^C_h)\}$, where the target tag set $T^C = \{t^C_1, ..., t^C_c\}$ differs from $T^F$, and $c$ represents the number of coarse-grained entity types.

Given a Coarse-grained input sequence $\mathbf X^C = \{x^C_1, ..., x^C_m\}$ of length $m$, this sequence is fed into the Fine-grained Model(FG-Model) as input and generates fine-grained probabilities.
Since the model generates contextual representations at the fine-grained level, a mapping is required to align them with coarse-grained representation for model training.
To achieve this, we employ the F2C (Fine-to-Coarse) mapping matrix $\mathbf M$ to convert fine-grained probabilities into coarse-grained ones by mapping the hierarchy between the two datasets.

% \begin{align}
% \mathbf{M} \in \mathbb{R}^{f \times c} \end{align}
The coarse-grained output probability is generated as follows:
\begin{align}
p^C(y^C_i|x^C_i) = p^F(y^F_i|x^C_i) \cdot \mathbf M
\end{align}
where $\mathbf M \in \mathbb R^{f \times c}$.
\noindent
We can train the model with the coarse-grained dataset by minimizing the following loss:
% 최종적으로 다음과 같은 loss를 최적화하는 식으로 구성된다:
\begin{align} \label{eq: coarse loss}
L_C = -\frac 1m \sum^m_{i=1} y_i^C \log p^C(y^C_i|x^C_i)
\end{align}

% -------------------------- Filtering부분 추가해야 함



% ---------------------------- 뺄 부분?
% 우리는 FG-NER을 해결하기 위해 low-resource FG-dataset과 기존에 존재하는 rich-resource CG-dataset을 동시에 모델 학습에 사용하는 방식을 제안한다. 기존 방식들과 달리, 우리는 FG와 CG dataset을 동시에 학습에 사용함으로써 데이터셋 사이에 존재하는 label hierarchy를 직접적으로 반영한다.
% 실제 모델 학습 시, FG-dataset은 기존 방식처럼 학습하나 CG-dataset으로 학습 시 Mapping matrix와 Filtering이 적용되는 과정 설명
% ----------------------------

\subsection{F2C Mapping Matrix} \label{F2C Mapping Matrix}
% In this section, we describe the process of creating the F2C Mapping Matrix.
The goal of the F2C mapping matrix is to map related types in the hierarchy for joint use of coarse-grained and fine-grained datasets together.
% FG와 CG entity types 매핑을 통해 여러 데이터셋을 동시에 사용하여 학습할 수 있도록 하는 방식이다.
With this collaborative training, the model can directly learn the relation between two types of datasets.

% 이러한 방식으로 모델을 학습함으로써 FG와 CG entity types 사이의 similarity 및 relationship을 직접적으로 반영할 수 있다.
We generate the mapping matrix using the following steps.
%  우리는 다음과 같은 step을 통해 F2C Matrix를 생성한다.
First, finetune the \texttt{PLM} with the coarse-grained dataset $\mathcal D^C$.
% 먼저, PLM을 coarse-grained dataset으로 튜닝한다.
The fine-tuned model predicts the corresponding coarse-grained type for fine-grained samples.
Second, we feed the fine-grained training samples $X^F$ into the fine-tuned model to obtain predictions $\hat {\mathbf Y}^C$ for coarse-grained entity types.
Finally, we can get fine-grained golden labels and corresponding coarse-grained predict ions for the fine-grained training samples as follows:
\begin{align}
 \mathcal D^F_{train} = \{(\mathbf X^F_1, \mathbf Y^F_1, \hat{\mathbf Y}^C_1), ..., (\mathbf X^F_l, \mathbf Y^F_l, \hat{\mathbf Y} ^C_l) \} 
\end{align}
where $\hat{\mathbf{Y}}^C = \{\hat{y}^C_1, ..., \hat{y}^C_n\}$ denotes a predicted coarse-grained entity sequence, $\forall \hat y^C_i, and  \hat y^C_j \in~T^C$.

We define an F2C mapping matrix $\mathbf M$ of size $f \times c$, initialized with zeros, where each element $M_{ij}$ represents the mapping between fine-grained entity type $t^F_i$ and coarse-grained entity type $t^C_j$.

% We initialize the F2C mapping matrix $~{\mathbf M \in \mathbb R^{f \times c}}$ with zeros and count the predicted occurrences between $\mathbf Y^F$ and $\hat {\mathbf Y}^C$ using the following scoring function:
% \begin{align}\label{equation 7}
% \mathbf M(i,j) = 0   % ,  \forall i \in \{1,..., f\}, \forall j \in \{1, ..., c\} 
% \end{align}
\begin{align}
\mathbf M_{ij} = \sum^l_{p=1} \sum^n_{q=1} \mathbb I(\mathbf Y^F_{p,q} = t^F_i) \cdot \mathbb I (\hat {\mathbf Y}^C_{p,q} = t^C_j)
\end{align}
\noindent
, where $\mathbf M_{ij}$ indicates the element at the $i$-th row and $j$-th column of the matrix, $\mathbb I(\cdot)$ is an indicator function.

% \sum^l_{p=1}\sum^n_{q=1} \mathbb I(y^F_{p,q} = t^F_i \text{ and } \hat y^C_{p,q} = t^C_j)
For each $\mathbf M_i$, we select the top-$k$ coarse-grained indices with the highest frequency, denoted as \texttt{top-indices}$_i$ = [$\text{top}_1, ..., \text{top}_k$]

% 그다음 각 $M(i)$에 대해, 가장 많이 예측된 k개의 
% 만 남긴다
% not in, are excluded, not included in
Then, we set the elements not in \texttt{top-indices}$_i$ to 0 using the following function:

$$
\mathbf M_{ij}= \begin{cases}
			\mathbf M_{ij}, & \text{if $j$ is in } \texttt{top-indices$_i$} \\
                0, & \text{otherwise}
        \end{cases}
$$

Finally, we normalize the probability distribution for each of $\mathbf M_i$.
% We finally conduct the probability distribution normalization for each of $\mathbf M_i$.
% 최종적으로 각 $M(i)$ 에 대해 probability distribution normalization을 진행한다
\begin{equation}
\begin{aligned}
\mathbf M_{ij} = \frac{\mathbf M_{ij}} {\sum^c_{j=1} \mathbf M_{ij}}, \\ 
\forall i \in \{  1,2,…,f\}, j \in \{1,2,…,c\} 
\end{aligned}
\end{equation}



\subsection{Inconsistency Filtering} \label{Inconsistency Filtering}
% In the previous section(\autoref{F2C Mapping Matrix}), we proposed the F2C mapping matrix that maps the representation between coarse-grained and fine-grained data, allowing the use of coarse-grained data in fine-grained classifier training.
% 이전 챕터의 F2C mapping matrix를 통해 유사한 fine-grained representations와 coarse-grained representations를 연관시켜줌으로써 FG-classifier를 보다 효과적으로 학습할 수 있음을 보았다. 
% 결과를 아직 보여주지 않았는데, "효과적으로 학습할 수 있음을 보였다"라고 써도 되나... 싶어서 다르게 써보았습니다. 추후 수정 필요하면 고치겠습니다.
% 이전 섹션이라는 말이 뭔가 이상한데 생각해보고 이 부분도 수정하겠습니다.

Since different annotators may have labeled the datasets with varying ***criteria, there are cases where certain coarse-grained entities can not be suitably assigned to specific fine-grained entity types.
% on different standards or guidelines / with varying criteria
Therefore, this inconsistency can cause an impact on the degradation of the model's performance.

To address this issue, we devise the inconsistency filtering method aimed at masking less relevant data to mitigate the noise of the training dataset.
The inconsistency filtering screens out noisy information from the coarse-grained dataset and selectively incorporates the relevant data that aligns with the fine-grained NER task.
This filtering method enables the dynamic and automatic inspection of suitable coarse-grained data for fine-grained entity types.
% Therefore, coarse-grained dataset이 가진 noisy information을 필터링하고 specific task에 맞는 적합한 데이터만 유동적으로(flexible? automatically?, dynamically?) 사용하는 방식인 Inconsistaent Label FIltering을 제안한다.
Figure \ref{fig: overall: b} illustrates the process of the inconsistency filtering.
% \autoref{fig: overall}(b) illustrates the process of generating and applying inconsistency filtering.

We filter out ambiguously labeled coarse-grained entities through the consecutive core steps:
% We proceed with the \textit{Inconsistency Filtering} through the following steps:
\begin{comment}
mislabeled
reliably labeled
consistent label mining
Distinguish between irrelevant and relevant entities
screened out, filtered out
[NLLB] Furthermore, models can easily learn spurious correlations that are not meaningful for the task itself
inspect, examine, find out
confused, obvious
reliable
cleaning
\end{comment}
% FIltering은 다음과 같은 순서로 수행된다.
First, we fine-tune the fine-grained model using a low-resource fine-grained dataset~$\mathcal D^F_{train}$, then generate fine-grained probabilities $\tilde p^F$ by applying softmax to the output of the tuned model.
Using the fine-grained probabilities and the F2C mapping matrix, we can convert the fine-grained probabilities into coarse-grained probabilities $\tilde p^C$.
Then we predict $\tilde y^C $ for each coarse-grained input $x^C$.
% A model, finetuned with the fine-grained dataset under the few-shot setting, predicts $\hat {\mathbf Y}^C$  for coarse-grained samples $\mathbb Y^C$.
% 먼저, few-shot FG-dataset으로 충분히 tune된 모델과 F2C Matrix를 사용해 CG-training samples $\mathbb Y^C$에 대한 예측값 $\hat {\mathbf Y}^C$을 생성한다:
\begin{align}
    \tilde y^C = \argmax \tilde p^C(y_i^C|x^C_i)
\end{align} 

% ------------------------------------------이부분 없어도 되는지 확인
% Therefore, we can build the coarse-grained dataset using the predicted values for each sample as follow:
% \begin{align}
% \mathcal D^C_{train} = \{ (\mathbf X^C_1, \mathbf Y^C_1, \hat{ \mathbf Y }^C_1), ...,  (\mathbf X^C_h, \mathbf Y^C_h, \hat{ \mathbf Y }^C_h)\}    
% \end{align},
% \noindent
% where $\hat {\mathbf Y}^C = \{ \hat y^C_1, ..., \hat y^C_m\}$.
% --------------------------------------------

% 만약 output \tilde y^C가 
% If the predicted output matches the actual label of the coarse-grained sample, we consider the given coarse-grained sample closely related to the fine-grained entity type.

If the model trained on the fine-grained dataset accurately produces the coarse-grained prediction $\tilde y^C$ that corresponds to the coarse-grained golden label, we consider that coarse-grained data to be well-aligned and relevant to the fine-grained category.
% If the coarse-grained prediction $\tilde y^C$ of the model trained on the fine-grained dataset matches the coarse-grained golden label $y^C$, we consider that coarse-grained data as important and relevant to fine-grained information.
% 만약 fine-grained dataset으로 학습된 모델의 coarse-grained predict가 실제 coarse-graind label과 일치하다면, 그 coarse-grained data는 FG-NER과 관련된 중요한 데이터라고 판단한다.
% ---------------------------------- 이부분 보류
% 따라서, 우리는 각 training sample에 대해 다음과 같은 Filter를 생성할 수 있다.
% $$
% \texttt{Filter}(x) = 
%     \begin{cases}
%         1, & \text{if $y^C_i = \hat{\mathbf y}^C_i$ }\\
%         0, & \text{otherwise}
%     \end{cases}
% $$
% ----------------------------------
% 우리는 실제 모델 학습 시, Filtering을 적용해 올바르게 예측된 Coarse-grained data만 학습에 반영한다.
Consequently, during the model training, we can exclusively leverage the accurately predicted coarse-grained data through inconsistent filtering.
% via / through / thanks to 
Finally, we revise Equation \ref{eq: coarse loss} as follows,
% Finally, 식 를 다음과 같이 수정한다:
\begin{align}
\tilde L_C = -\frac 1m \sum^m_{i=1} y_i^C \log p^C(y^C_i|x^C_i) \cdot \mathbb I [y^C_i = \tilde y ^C_i].
\end{align}
 
% The shared purpose of the two components is to give a single model two kinds of datasets for enhancing hierarchical connections.

% -------------------------------- 없앨 부분
%- [문단 1] CG-dataset에서 FG-entity types와 관련있는 정보만 추출할 수 있는 Filtering Method 제안
    % - coarse-grained dataset이 가진 데이터가 fine-grained entity types에 관련된 데이터인지 판단
% - [문단 2] coarse-grained dataset이 가진 noisy한 정보를 필터링하고, our purpose에 적합한 데이터만 유동적으로 사용

% \subsubsection{Filtering Procedure}
% In contrast to the F2C Matrix, we use a model fine-tuned with a fine-grained dataset in the inconsistent label filtering process.
% \begin{enumerate}
%   \item Train with model fine-tuned with a fine-grained dataset
%   \item filter
%   \item We only use unfiltered entities for the training phase
% \end{enumerate}

% 1. FG-dataset로 학습된 모델 사용
% 2. 학습된 모델이 mapping matrix를 통해 CG entity types를 올바르게 예측한 경우, 그 데이터는 FG-NER과 관련된 ~~중요한 데이터(clean data?)~~라고 판단
%     1. FG 학습에 이용가능한 applicable to FG/consistent with FG
% 3. 실제 모델 학습 시 올바르게 예측된 CG-data만 학습에 반영
% -----------------------------------
